Learning the Finer Things: Bayesian Structure Learning at the Instantiation Level

Successful machine learning methods require a trade-off between memorization and generalization. Too much memorization and the model cannot generalize to unobserved examples. Too much over-generalization and we risk under-fitting the data. While we commonly measure their performance through cross validation and accuracy metrics, how should these algorithms cope in domains that are extremely under-determined where accuracy is always unsatisfactory? We present a novel probabilistic graphical model structure learning approach that can learn, generalize and explain in these elusive domains by operating at the random variable instantiation level. Using Minimum Description Length (MDL) analysis, we propose a new decomposition of the learning problem over all training exemplars, fusing together minimal entropy inferences to construct a final knowledge base. By leveraging Bayesian Knowledge Bases (BKBs), a framework that operates at the instantiation level and inherently subsumes Bayesian Networks (BNs), we develop both a theoretical MDL score and associated structure learning algorithm that demonstrates significant improvements over learned BNs on 40 benchmark datasets. Further, our algorithm incorporates recent off-the-shelf DAG learning techniques enabling tractable results even on large problems. We then demonstrate the utility of our approach in a significantly under-determined domain by learning gene regulatory networks on breast cancer gene mutational data available from The Cancer Genome Atlas (TCGA).

==> Tables/keel-mdl-reduced.tex <==
\begin{table*}[ht]
\centering
\caption{A subset of \textit{Data} MDL results for BKBs learned with our BKB learning algorithm with GOBNILP DAG learning backend as well as BNs learned over same dataset with standard MDL scoring and GOBNILP. Also reported are the number of unique calls to the joint probability calculator for both BKB and BN learning. Results on several other datasets available in Appendix Table ~\ref{tab:mdl-results}.}
\begin{tabular}{lccccc}
\hline
Dataset           & BKB MDL          & BN MDL   & BKB Calls        & BN Calls & Calls Difference \\ \hline
newthyroid        & \textbf{-73}     & -462     & \textbf{1257}    & 7200     & -5943            \\
car               & \textbf{-994}    & -5976    & \textbf{20369}   & 40000    & -19631           \\
banana            & \textbf{-2047}   & -5929    & \textbf{103}     & 135      & -32              \\
saheart           & \textbf{-353}    & -1866    & \textbf{48005}   & 104976   & -56971           \\
mammographic      & \textbf{-300}    & -2126    & \textbf{2735}    & 6750     & -4015            \\
pima              & \textbf{-628}    & -3059    & \textbf{28309}   & 43740    & -15431           \\
tic-tac-toe       & \textbf{-1007}   & -4888    & \textbf{250986}  & 786432   & -535446          \\
ecoli             & \textbf{-199}    & -875     & \textbf{9044}    & 108864   & -99820           \\
contraceptive     & \textbf{-1060}   & -6083    & \textbf{194374}  & 1080000  & -885626          \\
yeast             & \textbf{-391}    & -4624    & \textbf{47816}   & 380160   & -332344          \\
titanic           & \textbf{-957}    & -2586    & \textbf{102}     & 108      & -6               \\
hayes-roth        & \textbf{-87}     & -403     & \textbf{928}     & 2000     & -1072            \\
iris              & \textbf{-69}     & -394     & \textbf{322}     & 1024     & -702             \\
bupa              & \textbf{-334}    & -760     & \textbf{1248}    & 2187     & -939             \\
haberman          & \textbf{-104}    & -384     & \textbf{80}      & 81       & -1               \\
glass             & \textbf{-155}    & -841     & \textbf{42539}   & 680400   & -637861          \\
phoneme           & \textbf{-1265}   & -13925   & \textbf{12389}   & 55440    & -43051           \\
tae               & \textbf{-65}     & -263     & \textbf{540}     & 972      & -432             \\
post-operative    & \textbf{-61}     & -319     & \textbf{16202}   & 184320   & -168118          \\
balance           & \textbf{-505}    & -1503    & \textbf{312}     & 324      & -12              \\
led7digit         & \textbf{-122}    & -1599    & \textbf{10204}   & 24057    & -13853           \\
monk-2            & \textbf{-229}    & -1548    & \textbf{6696}    & 8640     & -1944            \\ \hline
\end{tabular}
\label{tab:mdl-results-reduced}
\end{table*}

==> Tables/tcga-features.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccccc}
\hline
\multicolumn{5}{c}{TCGA Breast Cancer Features List}                                                                         \\ \hline
AHNAK                  & IRS4                   & CMYA5                    & CHD4                  & ERCC6                   \\
C10orf12               & TG                     & FAM186A                  & CBFB                  & MAP1A                   \\
RP11-407N17.3          & COL4A6                 & MYO18B                   & SCN8A                 & PKHD1L1                 \\
ERBB2-chr17:39723967   & FOXA1-chr14:37592256   & PIK3CA-chr3:179210291    & SCN10A                & CDH1-chr16:68810236     \\
ADGRG4                 & ERBB3                  & ASPM                     & TP53-chr17:7674945    & PCDH15                  \\
TP53-chr17:7675095     & MGAM                   & ADCY8                    & ITIH6                 & CACNA1A                 \\
TP53-chr17:7674220     & TP53-chr17:7673803     & USP34                    & PTPRD                 & FOXA1-chr14:37592035    \\
ANK3                   & TP53                   & SVIL                     & FAM47A                & UTP20                   \\
GOLGB1                 & SLIT2                  & ADAMTSL3                 & KAT6A                 & DNAH8                   \\
TNN                    & TP53-chr17:7674953     & WSCD2                    & LRP1                  & CEP170                  \\
TP53-chr17:7674250     & DYNC1H1                & EML5                     & MYH1                  & BIRC6                   \\
VPS13D                 & CEP192                 & TP53-chr17:7673802       & CSPP1                 & PIK3CA-chr3:179210192   \\
LYST                   & TDRD6                  & RYR1                     & HERC1                 & XKR4                    \\
NEB                    & SETDB1                 & CDH1-chr16:68738315      & DMXL2                 & COL6A3                  \\
PIK3CA-chr3:179218304  & CACNA1C                & COL11A1                  & DAB1-chr1:57015131    & HECW2                   \\
CIT                    & AKAP6                  & PRDM10                   & HDAC6                 & BRINP3                  \\
MYLK                   & SMG1                   & CACNA1E                  & TP53-chr17:7674950    & RGAG1                   \\
CSMD3                  & DMD                    & ITPR1                    & MUC4-chr3:195783008   & MTOR                    \\
NCOR1                  & TP53-chr17:7673767     & FBN1                     & MDN1                  & MYH9                    \\
PIK3CA-chr3:179218306  & SCN11A                 & KIF1B                    & SHANK1                & FAT4                    \\
RAPGEF6                & WDR17                  & ADGRV1                   & ATRX                  & DNAH10                  \\
TP53-chr17:7674947     & BRCA2                  & FLG                      & WDFY3                 & CKAP5                   \\
PKHD1                  & DST                    & MUC2                     & TP53-chr17:7673781    & GRIA3                   \\
RYR3                   & SPATA31D1              & PDE4DIP                  & CCNB3                 & PRRC2C                  \\
MUC4                   & TP53-chr17:7674292     & SAGE1                    & GRM4-chr6:34022043    & PIWIL1                  \\
SETD2                  & CD9-chr12:6235559      & MYT1L                    & PTEN                  & GPR179                  \\
MFAP5-chr12:8650521    & FGFR2-chr10:121498520  & NF1                      & GCC2                  & COL6A6                  \\
CNTNAP5                & PIK3CA-chr3:179203765  & CFH                      & NOTCH2                & SPATA31C1               \\
KDM5B                  & KMT2E                  & MAP3K1                   & KIAA2026              & LAMA3                   \\
FLG2                   & RAD54B                 & KRAS-chr12:25245350      & BRWD1                 & SPAG17                  \\
HUWE1                  & WDR87                  & PIK3CA-chr3:179218294    & PRKDC                 & TMEM67-chr8:93809963    \\
COL12A1                & CEP350                 & CCDC180                  & LOXHD1                & OTOGL                   \\
VPS13C                 & FCRL5                  & FAT1                     & PREX2                 & CNTLN                   \\
ITPR2                  & UNC79                  & CDH1                     & QSER1                 & HMCN1                   \\
MKI67                  & RUNX1                  & FLNA                     & SPHKAP                & ADAMTS20                \\
FMN2                   & RYR2                   & ALMS1                    & HRNR                  & FLNC                    \\
IGSF10                 & ATM                    & DCHS2                    & TENM2                 & RNF213                  \\
MUC17                  & TRIM50-chr7:73325571   & TP53-chr17:7674894       & MADD                  & THADA                   \\
THSD7B                 & SYNE1                  & DNAH9                    & ERBB2                 & DNAH11                  \\
ANKRD17                & NRXN2                  & HIST1H3B                 & C5orf42               & ADAMTSL1                \\
SPTA1                  & ZNF208                 & PIK3CA-chr3:179218303    & DNAH3                 & WNK3                    \\
RBMXL3                 & PCDH11X                & FOXA1                    & CH17-140K24.8         & PLXNA3                  \\
CUBN                   & CENPE                  & OTOF                     & RELN                  & LRP2                    \\
ZFPM2                  & SCN1A                  & FGFR2                    & THSD7A                & AKAP9                   \\
PIK3CA-chr3:179234297  & XIRP2                  & DNAH5                    & BAZ2B                 & IGHG1                   \\
DLC1                   & ANK1                   & FREM2                    & KIAA1210              & SRCAP                   \\
SCN2A                  & HERC2                  & KMT2C                    & SVEP1                 & AKT1                    \\
GATA3-chr10:8064095    & HTATSF1                & DBNL-chr7:44040806       & AKT1-chr14:104780214  & UNC13C                  \\
PIK3CA-chr3:179234169  & APC                    & NUP153                   & ATP7A                 & LRRIQ1                  \\
HIST1H3B-chr6:26031841 & USH2A                  & DENND4B                  & PCDH19                & SPTB                    \\
COL4A5                 & FOXA1-chr14:37592107   & DCHS1                    & CAD                   & KIF13A                  \\
ADCY9                  & TCHH                   & VPS13B                   & PIK3CA-chr3:179199690 & VCAN                    \\
TENM1                  & MACF1                  & EYS                      & PRUNE2                & AHNAK2                  \\
DOCK11                 & WDFY4                  & LRBA                     & ATP10A                & MEGF8                   \\
PCDHB12                & TANC2                  & COL5A3-chr19:9997417     & MYO10                 & TLN1                    \\
MYH7                   & NALCN                  & TP53-chr17:7673764       & TP53-chr17:7674229    & COL4A3                  \\
TP53-chr17:7670685     & SELP                   & UBR4                     & UHRF1BP1L             & VPS13A                  \\
PTPRF                  & GTF2IRD2-chr7:74822357 & TRPM6                    & MYO7A                 & MAP2                    \\
LAMA4                  & ABCA9                  & CDH23                    & PKD1L1                & MAGI1                   \\
YLPM1                  & ABCC9                  & CEP290                   & TP53-chr17:7673788    & HIVEP1                  \\
PIK3CA-chr3:179234286  & TAF1L                  & AHCTF1                   & COL22A1               & CAMSAP1                 \\
GRIN2B                 & CAMSAP2                & BRWD3                    & CSMD1                 & TP53-chr17:7674885      \\
TP53BP1                & HECW1                  & ERBB2-chr17:39724747     & SCN7A                 & CACNA1F                 \\
COL6A5                 & MYH10                  & ZFHX4                    & SCN9A                 & ABCA13                  \\
AFF2                   & HEG1                   & MYH14                    & TAF1                  & FBN3                    \\
SPATA31D5P             & CD163L1                & PCDHGB4-chr5:141389874   & FREM1                 & GREB1L                  \\
CREBBP                 & PLXNA2                 & FAM208B                  & RYR3-chr15:33662609   & SSPO                    \\
TP53-chr17:7674872     & DNAH12                 & NCOA6                    & GRID1                 & GRIK2                   \\
TP53-chr17:7675085     & TP53-chr17:7675088     & ABCA8                    & KIAA2022              & MYO5B                   \\
SETX                   & DNAH17                 & ZP4                      & SYNE2                 & DOCK2                   \\
LRP1B                  & CHD9                   & PCNT                     & KIAA2018              & REV3L                   \\
PLCH1                  & CHD7                   & RIMS2                    & SI                    & NINL                    \\
TEP1                   & REXO1L1P               & GOLGA6L10-chr15:82345024 & ATP10B                & PAPPA2                  \\
CHD6                   & ABCA12                 & MGA                      & PRRC2B                & CFTR                    \\
FAT3                   & MUC16                  & MUC5B                    & HCFC1                 & DYNC2H1                 \\
MXRA5                  & DNAH6                  & USP9X                    & AMER1                 & TP53-chr17:7675190      \\
DCC                    & UBR5                   & CACNA1B                  & ZNF536                & FAM47C                  \\
LCT                    & TRRAP                  & CENPF                    & TP53-chr17:7673537    & TNRC6B                  \\
MUC4-chr3:195783009    & MED12                  & PIK3CA-chr3:179221146    & KIF4A                 & KIF16B                  \\
SACS                   & PLCE1                  & CEP162                   & CDH20                 & FRAS1                   \\
F8                     & MRC1                   & CFAP47                   & COL4A4                & UTRN                    \\
KCNT2                  & TEX15                  & NBEAL1                   & TPR                   & RNF4-chr4:2514476       \\
CACNA1D                & HDLBP                  & ATAD2B                   & HYDIN                 & TBC1D25                 \\
F5                     & RANBP2                 & DNAH1                    & KIAA1109              & LRRC7                   \\
PIK3CA                 & TLR4                   & SHROOM2                  & PIK3CA-chr3:179218307 & OBSCN                   \\
SPTAN1                 & C2orf16                & CPS1                     & HECTD1                & DNAH7                   \\
SPTBN2                 & TOPBP1                 & ZNF462                   & ASXL3                 & PLEC                    \\
RIMS1                  & TP53-chr17:7675076     & NID1                     & HTT                   & ZAN                     \\
AK9                    & TP53-chr17:7673776     & NAV3                     & PTEN-chr10:87933148   & FCGBP                   \\
PCLO                   & SF3B1-chr2:197402110   & KMT2D                    & PMFBP1                & LAMA1                   \\
COL7A1                 & TTN                    & MYH8                     & UNC5D                 & GON4L                   \\
CCDC168                & ARFGEF1                & DNHD1                    & MAP2K4                & APOB                    \\
ANKRD11                & ITPR3                  & KAT6B                    & ANK2                  & PLCB4                   \\
ANKRD36                & ASTN1                  & CNTN1                    & FRMPD4                & MYO16                   \\
SGSM1                  & PDZD2                  & CSMD2                    & MROH2B                & FAT2                    \\
FBXW7-chr4:152350097   & KIAA1549L              & DNAH2                    & TNXB                  & SDK1                    \\
ALDOA-chr16:30065810   & TSHZ3                  & MYCBP2                   & SF3B1                 & PCNXL2                  \\
COL14A1                & FBXW7                  & NUP160                   & KIF1B-chr1:10352639   & DNM1P47-chr15:101764200 \\
RIF1                   & RP1                    & TP53-chr17:7674221       & ZDBF2                 & LAMA2                   \\
KIAA0430               & CADPS                  & PEG3                     & ARID1B                & CBLB                    \\ \hline
\end{tabular}
\end{table}
